FINGR: Learning Dexterous Hand Control for Real-World Rubik's Cube Solving

Manipulating a Rubik's Cube with a single dexterous hand is a challenging test of sustained, contact-rich control: the hand must execute successive layer turns while keeping the cube secure. Each turn requires some fingers to support the cube while others push a moving layer, release contact, and reset for the next move. To learn this coordination, we introduce FINGR (Future-supervised Interaction Network with Geometric Representations), a policy that combines finger-relative geometry with future interaction prediction. A shared point encoder expresses the cube relative to each fingertip and aggregates its points without depending on cubie indexing. Learned future tokens share the observation encoder and receive supervision for contact-force changes, layer-turn progress, and finger joint displacement at multiple time scales. The resulting representation conditions a flow policy that directly generates finger actions. On a real dexterous hand, our policy achieves 99.0% success over 300 turn attempts, compared with 79.7% for the base flow policy. Integrated with grasping and table-assisted regrasping, the policy solves all ten scrambled $2\times2\times2$ cubes in a mean complete-system time of approximately 137 seconds. The project website is available at https://www.lyt0112.com/projects/FINGR

==> tables/ablation.tex <==
Base Flow Policy & 82.7 $\pm$ 13.0 & 76.7 $\pm$ 3.1 & 19.7 $\pm$ 7.5 & 0.7 $\pm$ 0.6 & 79.7 $\pm$ 8.0 & 5.67 $\pm$ 0.14 \\
Local Geometry & 92.7 $\pm$ 5.8 & 92.7 $\pm$ 1.2 & 7.0 $\pm$ 1.7 & 0.3 $\pm$ 0.6 & 92.7 $\pm$ 2.3 & \best{5.24 $\pm$ 0.04} \\
\ours{} & \best{99.3 $\pm$ 1.2} & \best{98.7 $\pm$ 1.2} & \best{1.0 $\pm$ 1.0} & \best{0.0 $\pm$ 0.0} & \best{99.0 $\pm$ 1.0} & 5.25 $\pm$ 0.20 \\


==> tables/baseline.tex <==
ACT & 72.0 $\pm$ 8.7 & 83.3 $\pm$ 6.4 & 22.3 $\pm$ 6.5 & \best{0.0 $\pm$ 0.0} & 77.7 $\pm$ 6.5 & 6.39 $\pm$ 0.62 \\
Diffusion Policy & 78.0 $\pm$ 11.1 & 79.3 $\pm$ 13.0 & 20.3 $\pm$ 6.7 & 1.0 $\pm$ 0.0 & 78.7 $\pm$ 6.7 & 6.06 $\pm$ 0.14 \\
Base Flow Policy & 82.7 $\pm$ 13.0 & 76.7 $\pm$ 3.1 & 19.7 $\pm$ 7.5 & 0.7 $\pm$ 0.6 & 79.7 $\pm$ 8.0 & 5.67 $\pm$ 0.14 \\
\ours{} & \best{99.3 $\pm$ 1.2} & \best{98.7 $\pm$ 1.2} & \best{1.0 $\pm$ 1.0} & \best{0.0 $\pm$ 0.0} & \best{99.0 $\pm$ 1.0} & \best{5.25 $\pm$ 0.20} \\


==> tables/formulas.tex <==
1 & \texttt{R' F U2 R2 U2 R' F U' F R2 U2} & \texttt{UL2U3L3} / \texttt{LUL2ULU2L} \\
2 & \texttt{R' U2 F U F U' F R2 F' R U'} & \texttt{LU2LUL2} / \texttt{U3LULULUL} \\
3 & \texttt{U' F' R U2 R U' R2 U' F' U2 R} & \texttt{LU3L} / \texttt{L2ULU3} \\
4 & \texttt{U' R' U2 R' F U' F' U2 R U' R} & \texttt{LULU2L3UL} / \texttt{ULU2LULU2} \\
5 & \texttt{U R' F' R2 U2 R2 U' F U2 F' R2} & \texttt{LULULULUL3U2LULU} \\
6 & \texttt{U' R' U' F' U R' U2 R U2 F U2} & \texttt{LU} / \texttt{U2LUL2U2LULUL2} \\
7 & \texttt{U R' F U2 F2 R U' F' R U2 R'} & \texttt{U2L3UL} / \texttt{ULULU2L3UL3} \\
8 & \texttt{R U2 R2 U' R' U2 R' F U' R U'} & \texttt{U2LULUL} / \texttt{LULULULULU3L3} $\to$ \texttt{L3} \\
9 & \texttt{R' U' R U F U' R' U' F U2 F} & \texttt{ULU2} / \texttt{U2LU2LULUL2U2LU2} \\
10 & \texttt{R' F' R U2 R U' R' U' F U' F} & \texttt{LULU2L3U2LU} / \texttt{U2LULUL3ULUL2} \\


==> tables/rounds.tex <==
ACT & 0 & 66 & 76 & 29 & \best{0} & 71 & 7.29 & 6.76 & 7.02 \\
ACT & 1 & 68 & 88 & 22 & \best{0} & 78 & 6.69 & 6.05 & 6.37 \\
ACT & 2 & 82 & 86 & 16 & \best{0} & 84 & 6.04 & 5.54 & 5.79 \\
Diffusion Policy & 0 & 80 & 92 & 13 & 1 & 86 & 6.40 & 5.42 & 5.91 \\
Diffusion Policy & 1 & 66 & 80 & 26 & 1 & 73 & 6.30 & 6.08 & 6.19 \\
Diffusion Policy & 2 & 88 & 66 & 22 & 1 & 77 & 5.59 & 6.57 & 6.08 \\
Base Flow Policy & 0 & 70 & 74 & 27 & 1 & 72 & 5.65 & 5.74 & 5.69 \\
Base Flow Policy & 1 & 82 & 76 & 20 & 1 & 79 & 5.59 & 6.00 & 5.79 \\
Base Flow Policy & 2 & 96 & 80 & 12 & \best{0} & 88 & 5.30 & 5.74 & 5.52 \\
Local Geometry & 0 & 96 & 92 & 6 & \best{0} & 94 & 5.44 & 5.03 & 5.23 \\
Local Geometry & 1 & 96 & 92 & 6 & \best{0} & 94 & 5.30 & 5.26 & 5.28 \\
Local Geometry & 2 & 86 & 94 & 9 & 1 & 90 & 5.51 & \best{4.89} & 5.20 \\
\ours{} & 0 & \best{100} & \best{100} & \best{0} & \best{0} & \best{100} & 5.42 & 5.31 & 5.36 \\
\ours{} & 1 & \best{100} & 98 & 1 & \best{0} & 99 & \best{4.83} & 5.19 & \best{5.01} \\
\ours{} & 2 & 98 & 98 & 2 & \best{0} & 98 & 5.36 & 5.36 & 5.36 \\


==> tables/solve_components.tex <==
1 & 8.72 & 90.20 & 1.80 & 24.95 & 11.40 & 3.80 & 140.87 \\
2 & 8.85 & 132.00 & \best{0.00} & 39.05 & 10.61 & 3.08 & 193.59 \\
3 & 9.02 & 71.10 & 0.70 & 24.56 & 10.30 & 3.79 & 119.48 \\
4 & \best{8.06} & 91.10 & \best{0.00} & 25.85 & 12.96 & 3.66 & 141.62 \\
5 & 8.31 & \best{63.40} & \best{0.00} & \best{0.00} & \best{10.10} & \best{2.26} & \best{84.08} \\
6 & 9.24 & 69.70 & \best{0.00} & 40.43 & 11.38 & 3.40 & 134.14 \\
7 & 9.27 & 84.21 & \best{0.00} & 30.43 & 11.31 & 2.88 & 138.09 \\
8 & 8.93 & 87.40 & 2.30 & 29.18 & 13.70 & 5.58 & 147.09 \\
9 & 8.95 & 65.40 & 3.20 & 27.80 & 10.83 & 4.94 & 121.12 \\
10 & 8.46 & 94.50 & \best{0.00} & 27.60 & 12.16 & 3.49 & 146.23 \\


==> tables/solves.tex <==
1 & 8 & 10 & 6.30 & 3.98 & 5.01 & 1 & 1.56 & 140.87 \\
2 & 9 & 8 & 9.92 & 5.34 & 7.76 & 1 & 1.97 & 193.59 \\
3 & 7 & 5 & 5.69 & 6.26 & 5.93 & 1 & 1.55 & 119.48 \\
4 & 10 & 9 & 5.28 & 4.26 & 4.79 & 1 & 1.83 & 141.62 \\
5 & 8 & 9 & 3.35 & 4.07 & 3.73 & 0 & \best{0.50} & \best{84.08} \\
6 & 8 & 8 & 4.50 & 4.21 & 4.36 & 1 & 3.95 & 134.14 \\
7 & 8 & 12 & 4.29 & 4.16 & 4.21 & 1 & 3.10 & 138.09 \\
8 & 11 & 9 & 4.88 & 3.74 & 4.37 & 1 & 2.92 & 147.09 \\
9 & 13 & 7 & \best{3.18} & \best{3.43} & \best{3.27} & 1 & 2.90 & 121.12 \\
10 & 12 & 14 & 3.64 & 3.63 & 3.63 & 1 & 3.23 & 146.23 \\


==> tables/stages.tex <==
Pregrasp and initial planning & 10 / 10 & \best{100.0} & 3.33 $\pm$ 0.06 \\
Approach & 10 / 10 & \best{100.0} & 1.00 $\pm$ 0.00 \\
Grasp closure & 10 / 10 & \best{100.0} & 2.00 $\pm$ 0.05 \\
Lift and manipulation-pose rotation & 10 / 10 & \best{100.0} & 2.46 $\pm$ 0.41 \\
Planned layer turn & 181 / 185 & 97.8 & 4.59 $\pm$ 3.13 \\
Alignment & 4 / 4 & \best{100.0} & 2.00 $\pm$ 1.04 \\
Table-assisted regrasp & 9 / 9 & \best{100.0} & 29.98 $\pm$ 5.86 \\
Final placement and return & 10 / 10 & \best{100.0} & 11.48 $\pm$ 1.16 \\

